Finite-Time Analysis of Asynchronous Multi-Agent TD Learning

Recent research endeavours have theoretically shown the beneficial effect of cooperation in multi-agent reinforcement learning (MARL). In a setting involving $N$ agents, this beneficial effect usually comes in the form of an $N$-fold linear convergence speedup, i.e., a reduction - proportional to $N$ - in the number of iterations required to reach a certain convergence precision. In this paper, we show for the first time that this speedup property also holds for a MARL framework subject to asynchronous delays in the local agents' updates. In particular, we consider a policy evaluation problem in which multiple agents cooperate to evaluate a common policy by communicating with a central aggregator. In this setting, we study the finite-time convergence of \texttt{AsyncMATD}, an asynchronous multi-agent temporal difference (TD) learning algorithm in which agents' local TD update directions are subject to asynchronous bounded delays. Our main contribution is providing a finite-time analysis of \texttt{AsyncMATD}, for which we establish a linear convergence speedup while highlighting the effect of time-varying asynchronous delays on the resulting convergence rate.

==> ConvAnalCameraReady.tex <==
In this section, we prove Theorem \ref{th:main}. We start by introducing the following definitions to lighten the notation:
\begin{equation}\label{eq:dxddifftau}
\begin{aligned}
    \muiktau(\x) & \triangleq \|\E{\mathbf{g}_{i,k}(\x, \okn)|o_{i, k-\tau}} - \barg(\x)\|,\ k\geq \tau, \\
    \delta_{k, h} & \triangleq \|\x_{k} - \x_{k-h}\|,\ k\geq h\geq0,\\
    d_k &\triangleq \max_{k-2\tmax - \tau\leq j\leq k}\E{\delta_{j}^2},\ k\geq \tau + 2\tmax. 
\end{aligned}
\end{equation}
For our analysis, we will need the following result from \cite{bhandari2018}. 
%Specifically, the following Lemma contains the results provided in Lemma 1, 3 and 4 of \cite{bhandari2018}.
\begin{lemma}\label{lemma:bhand}
	The following holds $\forall \boldsymbol{\theta} \in \mathbb{R}^m$: 
\begin{equation*}\label{eq:bhandlemmas}
\begin{aligned}
		\langle \xs - \x, \barg(\x) \rangle \geq \omega(1-\gamma)\|\xs -\x\|^2.
\end{aligned}	
\end{equation*}
\end{lemma}\vspace{0.3cm}
We will also use the fact that the random TD update directions and their steady-state versions are 2-Lipschitz \cite{bhandari2018}, i.e., $\forall i \in [N], \forall k \in \mathbb{N}$, and $\forall \x, \x' \in \mathbb{R}^m$, we have: 
\begin{equation}\label{eq:Lipschitz}
\begin{aligned}
   \max\{\|\bfg(\x) - \bfg(\x')\|, \|\bar{\mathbf{g}}(\x) - \bar{\mathbf{g}}(\x')\| \} \leq 2\|\x - \x'\|.
\end{aligned}
\end{equation}
From \cite{srikant2019finite}, we also have that $\forall i \in [N], \forall k \in \mathbb{N},\forall \x\in \mathbb{R}^m$: 
\begin{equation}\label{eq:boundGradNorm}
    \|\mathbf{g}(\x, \okn)\|\leq 2\|\x\| + 2\bar{r},
\end{equation}
which, squared, using $\bar{r}\leq \sigma$, yields
\begin{equation}\label{eq:bGSq}
	\|\bfg(\x, o_{i,k})\|^2\leq 8(\|\x\|^2 + \sigma^2).
\end{equation}
We will often use the fact that, from the definition of the mixing time in Definition~\ref{def:mix}, we have, for a given iteration $k\geq\tau$, defining $\Theta_{i,k} \triangleq \{\x_{k-\tau}, o_{i,k-\tau}\}$,
\begin{equation}
	\label{eq:mixingProp}
	\Vert\mathbb{E}\left[\mathbf{g}(\boldsymbol{\theta}_{k-\tau}, o_{i,k})|\Theta_{i,k}\right]-\barg(\boldsymbol{\theta}_{k-\tau})\Vert \leq \alpha^{q}\left(\Vert \x_{k-\tau} \Vert +1 \right)
\end{equation}
The proof also relies on the following result from \cite{feyzmahdavian2014delayed}:
\begin{lemma}\label{lemma:OZDAG}
Let ${V_k}$ be non-negative real numbers that satisfy
\begin{align*}
	V_{k+1} &\leq p V_k + q \max_{(k-d(k))_+ \leq \ell \leq k} V_\ell+\beta,
\end{align*}
for $\beta,p,q>0$. Here, $k \geq 0$ and $0 \leq d(k) \leq d_{\max}$ for some $d_{\max}\geq0$. If $p+q<1$, then we have
\begin{align*}
	V_k \leq \rho^k V_0+\epsilon,
\end{align*}
where $\rho = (p+q)^{1/(1+d_{\max})}$ and $\epsilon=\frac{\beta}{1-p-q}$.
\end{lemma}
\noindent We will also use the fact that, for any $a, b \in \mathbb{R}, c\geq0$, 
\begin{equation}\label{eq:halfSq}
ab = a\sqrt{c}\frac{b}{\sqrt{c}} \leq \frac{1}{2}\pars{ca^2 + \frac{b^2}{c}},
\end{equation}
and also the  fact that, for $a_i\in\mathbb{R}, i = 1, ..., N$,
\eqal{eq:sumSqN}{
\pars{\sum_{i = 1}^{N}a_i}^2\leq N\sum_{i = 1}^{N}a_i^2.
}
Equipped with the above basic results, we now provide an outline of our proof before illustrating the technical details.

{\textbf{Outline of the proof}. Recall $t_{i, k} \triangleq \pars{k-\tau_{i,k}}_+$. We write the update rule \eqref{eq:updateRule} as
\eqal{}{
\xkp = \xk  + \alpha\vk = \xk + \alpha\barg(\xk) - \alpha \ek,
}
with $\ek \triangleq \barg(\xk) - \vk$. Thus, 
\eqal{}{
\ek = \frac{1}{N}\sum_{i = 1}^{N}\left(\barg(\xk) - \bfg(\x_{t_{i,k}}, o_{i, t_{i,k}})\right).
}
We analyze the following recursion:
\eqal{}{
\dxpd &= T_1+ \alpha^2T_2-2\alpha T_3 ,\hspace{0.2cm} \textrm{with}\\[4pt]
T_1 &= \|\xk - \xs + \alpha\barg(\xk)\|^2
\\[4pt]
T_2 &= \|\ek\|^2\\[4pt]
T_3 &= \langle \xk - \xs + \alpha \barg(\xk),\ek \rangle
.
}
The most important part of the proof consists of obtaining a bound of the following form:
\eqal{eq:desBound}{
\E{\dxpd} \leq p\E{\dxd} + O(\alpha^2(\tau+\tmax))d_k + B_{\alpha, N},
}
where $d_k$ was defined in \eqref{eq:dxddifftau}, $p<1$ is a contraction factor and
\eqal{}{
B_{\alpha, N} = O(\alpha^2(\tau + \tmax))\frac{\sigma^2}{N} + O(\alpha^4)\sigma^2,
}
which guarantees the linear speedup effect with $N$. The bound in \eqref{eq:desBound} allows us to obtain the desired result, by picking a step size small enough and applying Lemma \ref{lemma:OZDAG}. Given this outline, in the following we provide bounds for $\E{T_1}$, $\E{T_2}$ and $\E{T_3}$.

\textit{Bounding $\E{T_1}$.} Note that
\eqal{}{
T_1 &= \|\xk - \xs +\alpha\barg(\xk)\|^2
\\&= \dxd + 2\alpha\langle \xk - \xs,\barg(\xk) \rangle +\alpha^2\|\barg(\xk)\|^2.
}
Note that, using Lemma \ref{lemma:bhand}, we get
\eqal{}{
\langle \xk - \xs,\barg(\xk) \rangle &\leq -(1-\gamma)\omega\dxd,
}
and using~\eqref{eq:Lipschitz} we get
\eqal{}{
\|\barg(\xk)\|^2 &= \|\barg(\xk) - \barg(\xs)\|^2\leq 4\dxd.
}
Combining the two bounds above and taking the expectation,
\eqal{}{
\E{T_1} \leq (1-2\alpha(1-\gamma)\omega)\E{\dxd} + 4\alpha^2\E{\dxd}.
}

\textit{Bounding $\E{T_2}$.} We need the following result.
\begin{lemma}\label{lemma:boundvk}
For $k\geq \tau+ \tmax$, we have
\eqal{}{
\E{\|\vk\|^2}\leq 8\max_{k-\tmax\leq j\leq k}\E{\delta_j^2} + 32\frac{\sigma^2}{N} + 8\sigma^2\alpha^{2q}
}
\end{lemma}
\noindent Using the above Lemma, we are now in the position to proceed bounding $\E{T_2}$.
\eqal{}{
\E{T_2} = \E{\|\ek\|^2} &= \E{\|\barg(\xk) - \vk\|^2}
\\& \leq 2\E{\|\barg(\xk)\|^2 + \|\vk\|^2}.
}
Note that $\|\barg(\xk)\|^2 = \|\barg(\xk) - \barg(\xs)\|^2\leq 4\delta_k^2$, and so using Lemma \ref{lemma:boundvk} we get
\eqal{}{
\E{T_2}\leq 24\max_{k-\tmax\leq j\leq k}\E{\delta_j^2} + 64\frac{\sigma^2}{N} + 16\sigma^2\alpha^{2q}.
}

\textit{Bounding $\E{T_3}$.} We now bound $\E{T_3}$, which represents the major technical burden of the proof. 
We need the following result.
\begin{lemma}\label{lemma:delta_kh}
Let $k\geq \tmax + h$, {for some $h\geq0$}. Then,
\eqal{}{
\E{\delta_{k,h}^2}\leq 8\alpha^2h^2\pars{d_k + 4\frac{\sigma^2}{N} + \sigma^2\alpha^{2q}}
}
\end{lemma}
\noindent Equipped with the above results, we can prove the following further Lemma, that will enable us to complete the proof.
\begin{lemma}
    For 
\end{lemma}
\eqal{}{
T_3 &= K + T_{32}, \hspace{0.1cm} \textrm{with}
\\K &= \langle \xk - \xs,\ek \rangle, \\ T_{32} &=  \alpha\langle\barg(\xk), \ek\rangle.
}
Note that, using Cauchy-Schwarz and \eqref{eq:halfSq}, 
\eqal{}{
T_{32}&\leq \frac{\alpha}{2}\left(\|\barg(\xk)\|^2 + \|\ek\|^2\right)
\\&\leq 2\alpha\delta_k^2 + \frac{\alpha}{2}\|\ek\|^2.
}
Taking the expectation and using the bound on $\E{T_2}$,
\eqal{}{
\E{T_{32}}\leq  \alpha(14d_k + 32\frac{\sigma^2}{N} + 8\sigma^2\alpha^{2q}).
}
Now we bound $K$. Define $\barg_{N,k} \triangleq \frac{1}{N}\sum_{i = 1}^{N}\barg(\x_{k-\tau_{i,k}}).$
Adding and subtracting $\barg_{N,k}$, we write 
\eqal{}{
K &= K_1 + K_2, \hspace{0.3cm}\textrm{with}
\\
K_1 &= \inner{\xk - \xs}{\barg(\xk) - \barg_{N,k}},
\\
K_2 &= \inner{\xk-\xs}{\barg_{N,k} - \vk}.
}
Now note that, taking the sum of the second term outside of the inner product in $K_1$, 
\eqal{}{
K_1 &= \frac{1}{N}\sum_{i = 1}^{N}K_{1,i}, \hspace{0.3cm}\textrm{with}
\\K_{1,i} &= \inner{\xk-\xs}{\barg(\xk) - \barg(\x_{t_{i,k}})}.
}
We now bound $\E{K_{1, i}}$. Using \eqref{eq:halfSq} and \eqref{eq:Lipschitz},
\eqal{}{
{K_{1, i}} &\leq {\alpha\tmax}{\delta_k^2} + \frac{1}{4\alpha\tmax}{\|\barg(\xk) - \barg(\x_{t_{i,k}})\|^2}
\\&
\leq {\alpha\tmax}{\delta_k^2} + \frac{1}{\alpha\tmax}\delta_{k, \tau_{i,k}}^2.
}
Note that, using Lemma~\ref{lemma:delta_kh}, which requires $t_{i,k}= k-\tau_{i,k}\geq \tau$, which holds for $k\geq \tmax+\tau$,
\eqal{eq:deltaTau}{
\E{\delta_{t_{i,k}, \tau}^2}\leq 8\alpha^2\tmax^2\pars{d_k + 4\frac{\sigma^2}{N} + \sigma^2\alpha^{2q}}.
}
Taking the expectation and applying \eqref{eq:deltaTau}, we get
\eqal{}{
\E{K_{1,i}}\leq \alpha\tmax \pars{9d_k + 32\frac{\sigma^2}{N} + 8\sigma^2\alpha^{2q}},
}
and note that $\E{K_1}$ is bounded by the same quantity.
We now proceed to bound $\E{K_2}$. 
\eqal{}{
K_2 &= \frac{1}{N}\sum_{i = 1}^{N}K_{2,i}, \hspace{0.3cm}\textrm{with}
\\K_{2,i} &= \inner{\xk-\xs}{\barg(\x_{t_{i,k}}) -\dgit}
\\& = \Delta_{1,i} + \Delta_{2, i} + \Delta_{3, i},\hspace{0.3cm}\textrm{where}
\\[3pt]
\Delta_{1,i} &= \inner{\xk-\xs}{\barg(\x_{t_{i,k}}) - \barg(\x_{t_{i,k} -\tau})},
\\
\Delta_{2,i} &= \inner{\xk-\xs}{\barg(\x_{t_{i,k}-\tau}) - \bfg(\x_{t_{i,k} -\tau}, \odit)}
\\
\Delta_{3,i} &= \inner{\xk-\xs}{\bfg(\x_{t_{i,k} -\tau}, \odit) - \bfg(\x_{t_{i,k}}, \odit)}.
}
Note that, using Cauchy-Schwarz inequality and \eqref{eq:Lipschitz},
\eqal{eq:Delta1i}{
\Delta_{1,i}&\leq \delta_k\|\barg(\x_{t_{i,k}}) - \barg(\x_{t_{i,k}-\tau})\|
\\&
\leq 2\delta_k\delta_{t_{i,k}, \tau}
\\&
\overset{\eqref{eq:halfSq}}\leq \pars{\alpha\tau\delta_k^2 + \frac{\delta_{t_{i,k}, \tau}^2}{\alpha\tau}}.
}
For $k\geq \tau+\tmax$, we can apply Lemma~\ref{lemma:delta_kh} and get
\eqal{}{
\E{\delta_{t_{i,k}, \tau}^2}\leq \alpha^2\tau^2\pars{8d_k + 32\frac{\sigma^2}{N} + 8\sigma^2\alpha^{2q}}.
}
Thus, taking the expectation, we can get
\eqal{}{
\E{\Delta_{1, i}}\leq 9\alpha\tau d_k + 32\alpha\tau\frac{\sigma^2}{N} +8\alpha\tau\sigma^2\alpha^{2q}.
}
Note that, using the Lipschitz property (see~\eqref{eq:Lipschitz}), we get the exact same bound for $\Delta_{3, i}$. Now note that
\eqal{}{
K_2 &= \frac{1}{N}\sum_{i = 1}^{N}\pars{\Delta_{1, i} + \Delta_{3, i}} + \bar{\Delta},\hspace{0.3cm}\textrm{with}
\\
\bar{\Delta} &= \frac{1}{N}\sum_{i = 1}^{N}\Delta_{2, i}.
}
To bound $\bar{\Delta}$, we want to use the geometric mixing property of the Markov chain, that follows from Assumption \ref{assump:mixing}. However, due to the correlations existing between the iterates $\x_{t_{i,k}}$, this needs to be done with special care. Defining $k' \triangleq k-\tmax-\tau$, we start by adding and subtracting $\x_{k'}$ from the first term in the inner product of $\Delta_{2, i}$, getting 
\eqal{}{
\bar\Delta &= \bar{\Delta}_1 + \bar{\Delta}_2, \hspace{0.3cm}\textrm{with}
\\
\bar{\Delta}_1 &= \langle\xk-\x_{k'},\frac{1}{N}\sum_{i = 1}^{N}\barg(\x_{t_{i,k}-\tau}) -\dgitau\rangle,
\\
\bar{\Delta}_2 &= \langle\x_{k'} -\xs,\frac{1}{N}\sum_{i = 1}^{N}\barg(\x_{t_{i,k}-\tau}) -\dgitau\rangle.
}
Note that we can write, using~\eqref{eq:halfSq} and~\eqref{eq:sumSqN},
\eqal{}{
\bar{\Delta}_1&{\leq} \frac{1}{2\alpha\pars{\tmax+\tau}}\delta_{k, \tau+\tmax}^2 \\&+ \frac{\alpha\pars{\tmax+\tau}}{2N^2}\underbrace{\Vert\sum_{i = 1}^{N}\barg(\x_{t_{i,k}-\tau}) -\dgitau\Vert^2}_{G}
}
For $k\geq \tau+2\tmax$, we can apply Lemma~\ref{lemma:delta_kh} and get
\begin{equation}\label{eq:deltaTauMax}
\E{\delta_{k, \tau+\tmax}^2}\leq 8\alpha^2\pars{\tau+\tmax}^2(d_k + 4\frac{\sigma^2}{N} + \sigma^2\alpha^{2q}).
\end{equation}
Now note that
\eqal{}{
G\leq 2\underbrace{\|\sum_{i = 1}^{N}\barg(\x_{t_{i,k}-\tau})\|^2}_{G_{1}} + 2\underbrace{\|\sum_{i = 1}^{N}\dgitau\|^2}_{G_{2}},
}
with $\E{G_{1}}\leq 4N^2\E{\delta_{t_{i,k}-\tau}^2}\leq 4N^2d_k$. Also note that 
\eqal{}{
G_2 &\leq 2G_{21} + 2G_{22},\hspace{0.3cm} \textrm{with}
\\G_{21} & =  \|\sum_{i = 1}^{N}\dgitau - \bfg(\xs, o_{i, k-\tau_{i,k}})\|^2,
\\G_{22} & = \|\sum_{i = 1}^{N}\bfg(\xs, \odit)\|^2.
}
Note that $\E{G_{21}}$ and $\E{G_{22}}$ can be bounded in the same way as $\E{V_1}$ and $\E{V_2}$ in the proof of Lemma~\ref{lemma:boundvk}. We get
\eqal{}{
\E{G_{2}}\leq 8\pars{N^2d_k + 4N\sigma^2 + N^2\sigma^2\alpha^{2q}}.
}
Hence, we get
%\leq 4\alpha\pars{\tmax+\tau}\pars{d_k + 4\frac{\sigma^2}{N} + \sigma^2\alpha^{2q}}\\&+4\alpha\pars{\tmax +\tau}\pars{3d_k + 8\frac{\sigma^2}{N} + \sigma^2\alpha^{2q}}\\&
\eqal{}{
\E{\bar{\Delta}_1}&
\leq 16\alpha\pars{\tmax+\tau}\pars{d_k + 3\frac{\sigma^2}{N} +{\sigma^2\alpha^{2q}}}.
}
Defining $\bar{\Delta}_{2, i}\triangleq\langle\x_{k'} -\xs,\barg(\x_{t_{i,k}-\tau}) -\dgitau\rangle$,
\eqal{}{
\E{\bar{\Delta}_2} = &\frac{1}{N}\sum_{i = 1}^{N}\E{\bar{\Delta}_{2, i}}.
}
Now, defining $\bar{\Theta}_{i, k} \triangleq \{\x_{k'}, \x_{t_{i,k}-\tau}, o_{t_{i,k}-\tau}\}$,
\eqal{}{
\E{\bar{\Delta}_{2, i}} =& \mathbb{E}[\langle\x_{k'} -\xs,\barg(\x_{t_{i,k}-\tau}) -\dgitau\rangle]
\\
= &\mathbb{E}[\langle \x_{k'} -\xs, \\&\barg(\x_{t_{i,k}-\tau})-\E{\dgitau|\bar{\Theta}_{i, k}} \rangle]
\\
\leq& \mathbb{E}[\delta_{k'}
\\&\cdot\underbrace{\|\barg(\x_{t_{i,k}-\tau}) - \E{\dgitau|\bar{\Theta}_{i, k}}\|}_{\bar{\eta}_{k,i}}]
.
}
Now, recall $\Theta_{i, k} = \{\x_{t_{i,k}-\tau}, o_{i, t_{i,k}-\tau}\}$. Note that, for the memoryless property of the Markov chain $\{o_{i,k}\}$, we have
\eqal{}{
\E{\dgitau|\bar{\Theta}_{i, k}} = \E{\dgitau|\Theta_{i, k}}.
}
Indeed, by inspecting the update rule \eqref{eq:updateRule} we see that the parameter $\x_{k'}$ is a function of agent $i$ observations only up to time step $k'-1$, so up to observation $o_{i, k'-1}$. Hence, all the statistical information contained in $\x_{k'}$ has no influence on the random variable $o_{i,t_{i,k}}$ once we condition on $o_{i, t_{i,k}-\tau}$, because $t_{i,k}-\tau = k-\tau_{i,k}-\tau> k'-1= k-\tmax-\tau-1$. Therefore,
\eqal{}{
\bar{\eta}_{k,i} &= \|\barg(\x_{t_{i,k}-\tau}) - \E{\dgitau|{\Theta}_{i, k}}\|
\\&
\overset{\eqref{eq:mixingProp}}\leq \alpha^q\pars{\|\x_{t_{i,k} - \tau}\| + \sigma}.
}
Hence, we get
\eqal{}{
\E{\bar{\Delta}_{2, i}}&\leq \E{\delta_{k'}\alpha^q\pars{\|\x_{t_{i,k} - \tau}\| + \sigma}}
\\&
\leq \E{\delta_{k'}\alpha^q\pars{\delta_{t_{i,k}-\tau} + 2\sigma}}
\\&
\leq \E{\frac{\alpha}{2}\delta_{k'}^2 + {\alpha^{2q-1}}\pars{\delta_{t_{i,k}-\tau}^2 +4\sigma^2}}
\\&
\leq \alpha d_k + 4\alpha\sigma^2\alpha^{2\pars{q-1}}
\\&
\leq \alpha d_k + 4\alpha\sigma^2\alpha^{q}
}
where we used the fact that $\alpha\leq\frac{1}{2}$ and the fact that $2(q-1)\geq q$ for $q\geq2$.
Putting all the above bounds together, and also the fact that $\alpha\leq \frac{1}{16\pars{\tmax+\tau}}$ we get
\eqal{}{
\E{T_3}\leq \alpha\pars{\tmax+\tau}\pars{44d_k + 144\frac{\sigma^2}{N}} + 7\alpha\sigma^2\alpha^q.
}

\textit{Concluding the proof.} Using the bounds on $\E{T_1}, \E{T_2}$ and $\E{T_3}$, we obtain, for $k\geq \tau'\triangleq 2\tmax+\tau$,
\eqal{}{
\E{\dxpd}&\leq (1-2\alpha(1-\gamma)\omega)\E{\dxd}+15\alpha^2\sigma^2\alpha^q\\&+ \alpha^2\pars{\tau+\tmax}\pars{112d_k + 352\frac{\sigma^2}{N}}.
}
We can now write the above bound in the following way:
\eqal{}{
V_{k+1} &\red{\leq} pV_k + q\max_{k-\tau'\leq j\leq k}V_j + \beta,\hspace{0.2cm}\textrm{with}
\\V_k &= \E{\dxd},
\\p &= (1-2\alpha(1-\gamma)\omega),
\\q &= 112\alpha^2\pars{\tmax+\tau},
\\\beta &= 352\alpha^2\pars{\tmax+\tau}\pars{\frac{\sigma^2}{N}} + 15\alpha^2\sigma^2\alpha^q.}
Imposing $\alpha\leq \frac{(1-\gamma)\omega}{112(\tau+\tmax)}$, we get $p+q\leq 1 - \alpha(1-\gamma)\omega$, and we can apply Lemma~\ref{lemma:OZDAG} getting
\eqal{eq:aboveBound}{
\E{\delta_T^2}\leq \rho^{T-\tau'}\E{\delta_{\tau'}^2} + \epsilon,
}
with $\rho = \pars{1 - \alpha(1-\gamma)\omega}^{\frac{1}{1+\tau'}}$ and $\epsilon = \frac{\beta}{1-p-q}$. Note that we can easily show that $\rho^{-\tau'}\leq 2$ for $\alpha\leq \frac{1}{16(\tmax + \tau)}$. Furthermore, we can show that $\E{\delta_{\tau'}^2}\leq 3\sigma^2$, as we do next. Note that, using \eqref{eq:bGSq}, 
\eqal{}{
	\|\vk\|^2&\leq \frac{1}{N}\sum_{i = 1}^{N}8(2\delta_{t_{i,k}}^2 + 3\sigma^2)
	\\&
	\leq 16\max_{i = 1, ..., N}\delta_{t_{i,k}}^2 + 24\sigma^2.
}
Using this bound, note that, for any $k\geq 0$
\eqal{eq:formOf}{
	\delta_{k+1}^2 &= \delta_k^2 +2\alpha \langle \x_t - \xs,\vk \rangle + \alpha^2\|\vk\|^2
	\\&
	\overset{\eqref{eq:halfSq}}{\leq }\delta_k^2 + \alpha \delta_k^2 + \alpha\|\vk\|^2 + \alpha^2\|\vk\|^2
	\\&
	\leq (1+\alpha)\delta_k^2 + 2\alpha\|\vk\|^2
	\\&
	\leq (1+\alpha)\delta_k^2 + 32\alpha\max_{i = 1, ..., N}\delta_{t_{i,k}}^2  + 48\alpha \sigma^2,
}
where recall that $t_{i,k}\leq k$. Now define $\bar{p} \triangleq 1+\alpha$, $\bar{q} \triangleq 32\alpha$ and $\nu \triangleq \bar{p}+\bar{q}$ and $\bar{\beta} \triangleq48\alpha \sigma^2$. We now prove by induction that, for all $k\geq 0$, 
\eqal{eq:statAppIndBase}{
	\delta_k^2 \leq \nu^k\delta_{0}^2 + \epsilon_k,
}
where $\epsilon_k = \nu\epsilon_{k-1} + \bar{\beta}$ for $k\geq 1$ and $\epsilon_0 = 0$. The base case is trivially satisfied, because $\delta_0^2 \leq \delta_0^2$. As an inductive step, suppose that~\eqref{eq:statAppIndBase} is true for $0\leq s\leq k$, for some $k\geq 0$, so \eqal{}{
	\delta^2_s\leq \nu^s\delta^2_0 +\epsilon_s, \ \ \ 0\leq s\leq k.
}
Now, we check the property for $k+1$, using~\eqref{eq:formOf}, and noting that $\epsilon_k$ is an increasing sequence:
\eqal{}{
	\delta^2_{k+1} &\leq \bar{p}\delta_k^2 + \bar{q}\max_{i = 1, ..., N}\delta_{t_{i,k}}^2 + \bar{\beta},
	\\&
	\leq \bar{p}(\nu^k\delta^2_0 + \epsilon_k) + \bar{q}\pars{\max_{i = 1, ..., N}\nu^{t_{i,k}}\delta^2_0 + \epsilon_{t_{i,k}}} + \bar{\beta}
	\\&
	\leq \bar{p}(\nu^k\delta^2_0 + \epsilon_k) + \bar{q}(\nu^k\delta^2_0 + \epsilon_k) + \bar{\beta}
	\\&
	\leq (\bar{p}+\bar{q})\nu^k\delta^2_0 + (\bar{p}+\bar{q})\epsilon_k + \bar{\beta}
	\\&
	= \nu^{k+1}\delta^2_0 + \epsilon_{k+1}.
}
From which we can conclude the proof of~\eqref{eq:statAppIndBase}. Now, note that $\epsilon_k = \bar{\beta}\sum_{j = 0}^{k-1}\nu^j$,
and that for $0\leq k\leq {\tau}'$,
\eqal{}{
	\nu^k\leq \nu^{{\tau}'}\leq (1+33\alpha)^{{\tau}'}\leq e^{33\alpha{\tau}'}\leq e^{0.25}\leq 2,
}
imposing $\alpha\leq \frac{1}{132{\tau}'}$. Hence, for $0\leq k\leq {\tau'}$,
\eqal{}{
	{\delta_k^2}&\leq \nu^k\delta_0^2 + \epsilon_k\leq 2\delta_0^2 + \bar{\beta}\sum_{j = 0}^{{\tau'}-1}\nu^j\leq 2\delta_0^2 +2\bar{\beta} {\tau'} \\&= 2\delta_0^2 +2(48\alpha \sigma^2){\tau'}
	\leq 2\delta_0^2 + \sigma^2\leq 3\sigma^2,
}
where we used the fact that $\alpha\leq \frac{1}{100{\tau}'}$ and that $\delta_0^2 \leq \sigma^2.$ We can therefore conclude, writing the bound in \eqref{eq:aboveBound} as
\eqal{}{
\E{\delta_T^2}\leq \exp&\pars{-\frac{\alpha(1-\gamma)\omega T}{2\pars{\tau+\tmax}}}6\sigma^2 \\ &+ 352\frac{\alpha\pars{\tau+\tmax}\sigma^2}{\pars{1-\gamma}\omega N}
+ 15\frac{\alpha^3\sigma^2}{(1-\gamma)\omega}. 
}
\section{Simulations}
In this section, we provide simulation results to validate our theory. We consider an MDP with $|\mathcal{S}| = 100$ states and a feature space spanned by $d = 10$ orthonormal basis vectors; we set the discount factor to $\gamma = 0.5$ and the step size to $\alpha = 0.05$. To simulate the asynchronous delays in the TD update directions, we generate  random delays at each iteration $k$ for each agent $i$, by generating a uniform random variable $\tau_{i,k}$ in the range $[1, \tau_{max}]$. We set $\tau_{max} = 100$. In the multi-agent seting, we set the number of agents to $N = 20$. For each configuration, we plot the average of 20 experiments. From the results, it is apparent how the linear speedup property also holds for \texttt{AsyncMATD}. Furthermore, we can see how the gap between the delayed and non-delayed settings decreases in the multi-agent case, compared to the single-agent configuration, by more than one order of magnitude.
\begin{figure}[t]
\center
\includegraphics[width=0.75\columnwidth, trim ={0cm 0cm 0cm 0cm}, clip]{AsyncMATD_1.png}
	\caption{Comparison between vanilla \texttt{MATD} and \texttt{AsyncMATD} in single-agent ($N = 1$) and multi-agent ($N = 20$) settings. For \texttt{AsyncMATD}, we set $\tau_{max} = 100$.}
\label{fig:SimConst}
\end{figure}
\section{Conclusion and Future Work}
We presented and analysed \texttt{AsyncMATD}, providing the first finite-time analysis for asynchronous multi-agent TD learning that jointly establishes a linear convergence speedup with the number of agents. Future work includes more complex delay models, for example considering random and potentially unbounded delays. The analysis of these settings will require a careful study because the boundedness of the delays played a crucial role to prove our results. Future studies could also include analysing non-linear function approximation and studying the trade-off between using only a portion of the agents' updates - e.g., the set of agents whose transmissions are subject to the smallest delays~- instead of using all the available stale updates.


==> mainResult.tex <==
In this section, we state the main result of the paper in Theorem \ref{th:main} and provide a discussion on the meaning and implications. We provide a proof sketch with the main intuitions and insights on the key technical aspects, while the complete proof is illustrated in section \ref{sec:convergence}. First, we provide some preliminaries, starting with the following assumption:
\newtheorem{assumption}{Assumption}
\begin{assumption}\label{th:ass_1}
The Markov chain $\{o_{k, n}\}$ is aperiodic and irreducible.
\end{assumption}

Existing finite-time analysis of TDL with Markovian sampling use the fact that the Markov chain mixes exponentially fast, which is a consequence of Assumption \ref{th:ass_1} (see \cite{srikant2019finite, bhandari2018}). Given a parameter $\x$, we define 
\begin{equation}
    \muiktau(\x) \triangleq \|\E{\mathbf{g}(\okn, \x)|o_{k-\tau, n}} - \barg(\x)\|,
\end{equation}
and Assumption \ref{th:ass_1} implies that 
\begin{equation}
    \muiktau(\x)\leq m\rho^{\tau}(1 + \|\x\|),
\end{equation}
for all $n$ and for some positive constants $m$, $\rho < 1$. 

For all $\x, n$ the pseudo-gradient norm can be bounded in the folowing way (see \cite{srikant2019finite}):
\begin{equation}\label{eq:boundGradNorm}
    \|\mathbf{g}(\x, \okn)\|\leq \|\x\| + b_{max},
\end{equation}
with $b_{max}$ a positive constant. We define 
\begin{equation}
    \sigma \triangleq \text{max}\{b_{max},\  \|\xs\|\}.
\end{equation}
For notation convenience, we also define 
\begin{equation}
    \delta_k \triangleq \|\xk - \xs\|.
\end{equation}
\begin{theorem}\label{th:main}
	Consider the update rule (\ref{eq:OtA_TD}). There exist absolute constants $C, {C}'$ such that the following holds. Let
	\begin{equation}
		\alpha_{\tau} \leq \frac{\omega(1-\gamma)}{C\tau}.
	\end{equation}
	Fix $q \geq 2$ such that, for some $\tau'>0$, $\alpha_{\tau'}^{q} \leq 1/N$. Pick $\tau \geq \tau'$ large enough such that, $\forall{n, k, \x}$, 
	\begin{equation}\label{eq:muBound}
		\muiktau(\x) \leq \alpha_{\tau}^{q}(1 + \|\x\|).
	\end{equation}
The TD updates after $k\geq 2\tau$ iterations satisfy
\begin{equation}
	\E{\dxd} \leq (1 - \alpha_{\tau}\omega(1-\gamma)p)^{k-2\tau}\E{\delta^2_{2\tau}} + \frac{{C}'\alpha_{\tau}\tau\sigma^2}{\omega(1-\gamma)N}
\end{equation}
\end{theorem}

\textbf{Proof sketch:}

\textbf{Discussion:}
